Pragmatics of Formally Verified Yet Efficient Static Analysis, in particular for Formally Verified Compilers

Formally verified compilers and formally verified static analyzers are a solution to the problem that certain industries face when they have to demonstrate to authorities that the object code they run truly corresponds to its source code and that it satisfies certain properties. From a scientific and technological point of view, they are a challenge: not only a number of nontrivial invariants and algorithms must be proved to be correct, but also the implementation must be reasonably effective so that the tools operate within reasonable time. Many optimizations in compilers rely on static analysis, and thus a formally verified compiler entails formally verified static analyses.In this article, we explain some difficulties, possible solutions, design choices and trade-offs pertaining to verified static analysis, in particular when the solution of the analysis is expressed as some form of tree, map or set.

==> preamble__1_.tex <==
%%%% Standard Packages
%%<additional latex packages if required can be included here>

\usepackage{amsmath}
\usepackage{paralist}
\usepackage{graphicx}
%\usepackage{amsthm}
\usepackage{txfonts}
%\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
\usepackage{xcolor}%
%\usepackage{textcomp}%
\usepackage{manyfoot}%
%\usepackage{booktabs}%
%\usepackage{algorithm}%
%\usepackage{algorithmicx}%
%\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{hyperref}
%%%%

\lstset{basicstyle=\tt}

\lstdefinelanguage{Coq}{
%
% Anything betweeen $ becomes LaTeX math mode
mathescape=true,
%
% Comments may or not include Latex commands
texcl=false, 
%
% Vernacular commands
morekeywords=[1]{Section, Module, End, Require, Import, Export,
  Variable, Variables, Parameter, Parameters, Axiom, Hypothesis,
  Hypotheses, Notation, Local, Tactic, Reserved, Scope, Open, Close,
  Solve, Obligations,% Bind,
  Delimit, Extract, Inlined, Constant,
  Definition, Let, Ltac, Fixpoint, CoFixpoint,% Add,
  Morphism, Relation, Implicit, Arguments, Unset, Contextual,
  Strict, Prenex, Implicits, Inductive, CoInductive, Record,
  Structure, Canonical, Coercion, Context, Class, Global, Instance,
  Program, Infix, Theorem, Lemma, Corollary, Proposition, Fact,
  Remark, Example, Proof, Goal, Save, Qed, Defined, Hint, Resolve,
  Rewrite, View, Search, Show, Print, Printing, All, Eval, Check,
  Projections, inside, outside, Def},
%
% Gallina
morekeywords=[2]{forall, exists, 
exists2, fun, fix, cofix, struct,
  match, with, end, as, in, return, let, if, is, then, else, for, of,
  nosimpl, when},
% Sorts
morekeywords=[3]{Type, Prop, Set},
%
%
% Comments delimiters, we do turn this off for the manual
morecomment=[s]{(*}{*)},
%
% Spaces are not displayed as a special character
showstringspaces=false,
%
% String delimiters
morestring=[b]",
morestring=[d],
%
% Size of tabulations
tabsize=3,
%
% Enables ASCII chars 128 to 255
extendedchars=false,
%
% Case sensitivity
sensitive=true,
%
% Automatic breaking of long lines
breaklines=false,
%
% Default style fors listings
%basicstyle={\scriptsize\ttfamily},
%
% Position of captions is bottom
%captionpos=b,
%
% columns
%columns=[c]fixed,
%
%frame=single,
%
% Style for (listings') identifiers
%identifierstyle={\ttfamily},
% Style for declaration keywords
%keywordstyle=[1]{\ttfamily\bfseries\color{magenta}},
% Style for gallina keywords
%keywordstyle=[2]{\ttfamily\bfseries\color{blue}},
% Style for sorts keywords
%keywordstyle=[3]{\ttfamily\bfseries},
% Style for strings
%stringstyle=\ttfamily,
% Style for comments
%commentstyle={\ttfamily\color{red}\itshape},
%
%moredelim=**[is][\ttfamily\color{red}]{/&}{&/},
literate=
    {.}{{.}}0
    {:=}{{$\coloneqq$}}1
    {forall}{{$\forall$}}1
    {exists}{{$\exists$}}1
    {<-}{{$\leftarrow$}}1
    {=>}{{$\Rightarrow$}}2
    {<=}{{$\!\leq\!$}}1
    {>=}{{$\!\geq\!$}}1
    {==}{{\code{==}}}1
    {==>}{{\code{==>}}}1
%    {:>}{{\code{:>}\;}}1
    {->}{{$\rightarrow$}}1
    {~>}{{$\leadsto$}}1
    {~~>}{{$\leadsto$}}1 % TODO?
    {<~}{{$\leftsquigarrow$}}1
    {<->}{{$\leftrightarrow\;$}}1
%    {<==}{{$\leq\;$}}1
%    {\#}{{$^\star$}}1 
%    {\\o}{{$\circ\;$}}1 
%    {\@}{{$\cdot$}}1 
    {\/\\}{{$\wedge$}}1
    {\\\/}{{$\vee$}}1
    {++}{{\code{++}}}1
%    {\@\@}{{$@$}}1
%    {\\mapsto}{{$\mapsto\;$}}1
% in comments
%    {\\hline}{{\rule{\linewidth}{0.5pt}}}1
    {...}{{${\ldots}$}}1
%
}[keywords,comments,strings]

\lstnewenvironment{lstcoq}{\lstset{language=Coq,basicstyle={\smalllistingsize\tt}}}{}

\newcommand{\true}{\textsf{true}}
\newcommand{\false}{\textsf{false}}

\newcommand{\filename}[1]{\texttt{#1}}
\newcommand{\fileurl}[2]{\href{#1}{\filename{#2}}}
\newcommand{\filen}[2]{\fileurl{https://github.com/AbsInt/CompCert/blob/2ca39a2801d333abcfa3d691620d03abde4e7e37/#1/#2}{#2}}
\newcommand{\filenc}[2]{\fileurl{https://gricad-gitlab.univ-grenoble-alpes.fr/certicompil/Chamois-CompCert/-/blob/7544c6b9a71459799984059bdfb2029ccf992b44/#1/#2}{#2}}

\title{Pragmatics of Formally Verified Yet Efficient Static Analysis, in particular for Formally Verified Compilers}
\author{David Monniaux}

